ALIEN: Analytic Latent Watermarking for Controllable Generation

Watermarking is a technical alternative to safeguarding intellectual property and reducing misuse. Existing methods focus on optimizing watermarked latent variables to balance watermark robustness and fidelity, as Latent diffusion models (LDMs) are considered a powerful tool for generative tasks. However, reliance on computationally intensive heuristic optimization for iterative signal refinement results in high training overhead and local optima entrapment.To address these issues, we propose an \underline{A}na\underline{l}ytical Watermark\underline{i}ng Framework for Controllabl\underline{e} Generatio\underline{n} (ALIEN). We develop the first analytical derivation of the time-dependent modulation coefficient that guides the diffusion of watermark residuals to achieve controllable watermark embedding pattern.Experimental results show that ALIEN-Q outperforms the state-of-the-art by 33.1\% across 5 quality metrics, and ALIEN-R demonstrates 14.0\% improved robustness against generative variant and stability threats compared to the state-of-the-art across 15 distinct conditions. Code can be available at https://anonymous.4open.science/r/ALIEN/.

==> table/relatedwork.tex <==
\begin{table}[htbp]
    \centering
    \caption{Comparison of Watermarking Techniques}
    \label{tab:watermarks_comparison}
    \begin{tabular}{@{}lccc@{}} % @{} removes padding from the far left and right
        \toprule % Top thick rule
        \textbf{Watermark} & \textbf{Publication} & \textbf{Target Component} & \textbf{Extraction Mechanism} \\
        \midrule % Middle rule below the header
        StableSig. \cite{fernandez2023stable} & ICCV 2023 & VAE-Decoder & Watermark Decoder \\
        Tree-ring \cite{wen2024tree} & NeurIPS 2023 & $Z_T$ & Diffusion Inversion \\
        RingID \cite{ci2025ringid} & ECCV 2024 & $Z_T$ & Diffusion Inversion \\
        StegaStamp \cite{tancik2020stegastamp}& CVPR 2020 & $X_0$ & Watermark Decoder \\
        WaDiff \cite{min2024watermark}& ECCV 2024 & U-Net & Watermark Decoder \\
        PRC \cite{gunn2024undetectable} &ICLR 2025 & $Z_T$ & Diffusion Inversion\\
        Gaussian Shading \cite{yang2024gaussian} & CVPR 2024 & $Z_T$ & Diffusion Inversion\\
        Aqualora \cite{feng2024aqualora} & ICML 2024 & U-Net & Watermark Decoder\\
        Sleepermark \cite{wang2025sleepermark} & CVPR 2025 & Prompt-U-Net & VAE-Encdoer+ Watermark Decoder\\
        RosteALS \cite{bui2023rosteals} & CVPR 2023 & $Z_0$ & Watermark Decoder\\
        WOUAF \cite{kim2024wouaf} & CVPR 2024 & VAE-Decoder & Watermark Decoder\\
        Zodiac \cite{zhang2024attack} & NeurIPS 2024 & $Z_T$ & Diffusion Inversion \\
        MDDM \cite{xumddm} & ICML 2025 & $Z_T$ & Diffusion Inversion \\
        GaussMarker \cite{li2025gaussmarker} & ICML 2025 & $Z_T$ & Diffusion Inversion \\
        Lawa \cite{rezaei2024lawa} & ECCV 2024 & VAE & Watermark Decoder \\
        Robin \cite{huang2024robin} & NeurIPS 2024 & $Z_t$ & Diffusion Inversion\\
        Shallow Diffuse \cite{lishallow} & NeurIPS 2025 & $Z_t$ &  Diffusion Inversion \\
        Obj-wm\cite{devulapally2025your} & ICCV 2025 & Token-UNet $$ & Watermark Decoder\\
        FSwatermark \cite{xiong2023flexible} & MM 2023 & VAE & Watermark Decoder\\
        WMAdapter \cite{ci2024wmadapter} & ICML 2025 & VAE & Watermark Decoder\\
        SEAL \cite{arabi2025seal} & ICCV 2025 & $Z_T$ & Diffusion Inversion\\
        Distrimark \cite{lei2025secure} & IJCAI 2025 & $Z_T$ & Diffusion Inversion + Watermark Decoder\\
        \bottomrule % Bottom thick rule
    \end{tabular}
\end{table}
